Simplifying Contract-Violating Traces

Contract conformance is hard to determine statically, prior to the deployment of large pieces of software. A scalable alternative is to monitor for contract violations post-deployment: once a violation is detected, the trace characterising the offending execution is analysed to pinpoint the source of the offence. A major drawback with this technique is that, often, contract violations take time to surface, resulting in long traces that are hard to analyse. This paper proposes a methodology together with an accompanying tool for simplifying traces and assisting contract-violation debugging.

==> eptcsdata.tex <==
\providecommand{\firstpage}{11}
\providecommand{\publicationstatus}{G. J. Pace and A. P. Ravn: \\
Proceedings of Sixth Workshop on Formal Languages\\
and Analysis of Contract-Oriented Software (FLACOS'12)\\
EPTCS 94, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.94.2}{10.4204/EPTCS.94.2}}
\pdfoutput=1

